Unraveling Instance Associations: A Closer Look for Audio-Visual Segmentation

Audio-visual segmentation (AVS) is a challenging task that involves accurately segmenting sounding objects based on audio-visual cues. The effectiveness of audio-visual learning critically depends on achieving accurate cross-modal alignment between sound and visual objects. Successful audio-visual learning requires two essential components: 1) a challenging dataset with high-quality pixel-level multi-class annotated images associated with audio files, and 2) a model that can establish strong links between audio information and its corresponding visual object. However, these requirements are only partially addressed by current methods, with training sets containing biased audio-visual data, and models that generalise poorly beyond this biased training set. In this work, we propose a new cost-effective strategy to build challenging and relatively unbiased high-quality audio-visual segmentation benchmarks. We also propose a new informative sample mining method for audio-visual supervised contrastive learning to leverage discriminative contrastive samples to enforce cross-modal understanding. We show empirical results that demonstrate the effectiveness of our benchmark. Furthermore, experiments conducted on existing AVS datasets and on our new benchmark show that our method achieves state-of-the-art (SOTA) segmentation accuracy.

==> algorithm/vpo_generation.tex <==

% \begin{algorithm}[h]
% \caption{Attribute to Sample Aggregation (A2S)}
% \label{alg:gr}
% \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
% \definecolor{codekw}{rgb}{0.85, 0.18, 0.50}
% \definecolor{ao}{rgb}{0.0, 0.5, 0.0}

\newcommand{\seg}{\text{seg}}
\newcommand{\vgg}{\text{vgg}}
\newcommand{\vpo}{\text{vpo}}
\newcommand{\snd}{\text{snd}}


\begin{algorithm}[!t]
\caption{VPO Generation Process}
\label{alg:vpo}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\definecolor{codekw}{rgb}{0.85, 0.18, 0.50}
\definecolor{ao}{rgb}{0.0, 0.5, 0.0}

\begin{algorithmic}[1]
    \State \textbf{require:} \\
    COCO dataset $\mathcal{D}_{\seg}=\{(\mathbf{x}_{\seg}, \mathbf{m}_{\seg}, \mathbf{y}_{\seg})_i\}_{i=1}^{|\mathcal{D}_{\seg}|}$, \\
    VGGSound dataset $\mathcal{D}_{\snd}=\{(\mathbf{a}_{\snd}, \mathbf{y}_{\snd})_i\}_{i=1}^{|\mathcal{D}_{\snd}|}$ dataset, where $\mathbf{y}_{\seg} \in \mathcal{Y}_{\seg}$ and $\mathbf{y}_{\snd} \in \mathcal{Y}_{\snd}$
    \State Create VPO dataset $\mathcal{D}_{\vpo}=\emptyset$.
    \State \textcolor{ao}{\# Dataset Preparation}
    \For{$(\mathbf{x}_{\seg}, \mathbf{m}_{\seg}, \mathbf{y}_{\seg})$ in $\mathcal{D}_{\seg}$} 
    \State \textcolor{codeblue}{\# Find intersections and filter out single objects}
    \State \textbf{If} $\mathbf{y}_{\seg} \in \mathcal{Y}_{\snd}$ and $|\mathsf{unique}(\mathbf{y}_\seg)| > 1$
    \State \textbf{Then} $(c_h, c_w) \leftarrow f_{\mathsf{centerofmass}}(\mathbf{m}_{\seg})$
    \State \hspace{\algorithmicindent}\hspace{6pt} $\alpha \leftarrow c_w/W$
    \State \hspace{\algorithmicindent}\hspace{6pt} 
    $\mathcal{D}_{\vpo} \leftarrow \mathcal{D}_{\vpo} \cup \{\mathbf{x}_{\seg}, \mathbf{m}_{\seg}, \mathbf{y}_{\seg}, \mathbf{a}_{\snd}, \alpha\}$
    \State \hspace{\algorithmicindent}\hspace{6pt} $\mathcal{D}_{\snd}\leftarrow\mathcal{D}_{\snd}-\{\mathbf{a}_{\snd}, \mathbf{y}_{\snd}\}$
    \EndFor
    \State \textbf{If} setting is VPO-SS \textbf{then}
    \State Filter out multi-source and multi-instance samples.
    \State \textbf{If} setting is VPO-MS \textbf{then}
    \State Filter out multi-instance samples.
    \State \textbf{If} setting is VPO-MSMI \textbf{then}
    \State Keep all samples.

    
    %\State \textbf{initial:} clean set $\mathcal{A}=\emptyset$ and noisy set $\mathcal{B}=\emptyset$

\end{algorithmic}
\end{algorithm}


==> dataset_compare.tex <==

% \begin{table}[t]
% \begin{center}
% % \vspace{-1mm}
% \caption{\textbf{Existing audio-visual dataset statistics.}}
% % \begin{tabular}{l rrrr}
% \setlength{\tabcolsep}{6pt}
% \resizebox{1\linewidth}{!}{  
% \begin{tabular}{cccccc}
% \toprule[0.8pt]\noalign{\smallskip}


\begin{table*}
\centering
\caption{Comparison of recently published AVS datasets~\cite{hu2022mix,zhou2022audio} and our proposed 
VPO-SS, VPO-MS, and AVSBench-Single+ benchmark datasets, in terms of the number of samples, number of classes, sample type, annotation type, and if the audio-visual samples are synthesised.}
% \resizebox{1.\linewidth}{!}{%
\begin{tabular}{!{\vrule width 1.5pt}cccccc!{\vrule width 1.5pt}} 
\specialrule{1.5pt}{0pt}{0pt}

Benchmark & \# Samples & Classes & Types  &  Annotations & Synthesised?\\
% \noalign{\smallskip}
\specialrule{1.5pt}{0pt}{0pt}
% VGG-SS~\cite{chen2021localizing}         & \,\,\,5,158  & 220  & Image & BBox (Saliency)    \\  
VGG-Instruments~\cite{hu2022mix} & \,\,\,446  & \,\,\,37  & Image+Audio & Binary (Pixel) & \textcolor{red}{\pmb{\tikzxmark}}          \\
AVSBench-S4~\cite{zhou2022audio}        & 10,852 & \,\,\,23   & Video & Binary (Pixel) & \textcolor{red}{\pmb{\tikzxmark}}              \\
AVSBench-MS3~\cite{zhou2022audio}        & 2,120 & \,\,\,23   & Video & Binary (Pixel) & \textcolor{red}{\pmb{\tikzxmark}}              \\
\rowcolor{LightCyan} VPO-SS & 12,202 & \,\,\,21   & Image+Audio & Multi-class (Pixel) & \textcolor{red}{\pmb{\tikzcmark}}               \\
\rowcolor{LightCyan} VPO-MS & 9,817 & \,\,\,21   & Image+Audio & Multi-class (Pixel) & \textcolor{red}{\pmb{\tikzcmark}}                \\
\rowcolor{LightCyan} AVSBench-Single+ & 10,852 & \,\,\,23   & Image+Audio & Multi-class (Pixel) & \textcolor{red}{\pmb{\tikzxmark}}     \\
\specialrule{1.5pt}{0pt}{0pt}
\end{tabular}
% }
\label{tab:comparison_with_datasets}
\vspace{-10pt}
\end{table*}



% \bottomrule[0.8pt]
% \end{tabular}
% }
% \end{center}
% \vspace{-8mm}
% \end{table}

==> table/ablation_ca.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|}
    \hline
        ~ & mIoU & F-beta & FDR \\ \hline
        Channel-wise & ~ & ~ & ~ \\ \hline
        Softmax & ~ & ~ & ~ \\ \hline
        min-max & ~ & ~ & ~ \\ \hline
        Sigmoid & ~ & ~ & ~ \\ \hline
    \end{tabular}
\end{table}

==> table/ablation_components.tex <==
% \begin{table*}[t!]
%     \centering
%     % \resizebox{1\textwidth}{!}{  
%     \begin{tabular}{c|c|c|cccc}														
% \thickhline														
% \toprule														
% Method	&	Backbone	&	Seg Model	&	FDR  $\downarrow$	&	mIoU $\uparrow$	&	F1 $\uparrow$	&	ACC $\uparrow$	\\	\midrule 
% Baseline	&	\multirow{3}{*}{ResNet50}	&	\multirow{3}{*}{DeepLabV3+}	&	15.56	&	68.11	&	80.37	&	94.24	\\	
% Cross attention	&	~	&	~	&	15.50	&	70.33	&	82.06	&	94.42	\\	
% CTR	&	~	&	~	&	12.71	&	74.17	&	84.86	&	95.15	\\	
% \bottomrule		%	-	-	-	-	-	-	-	-	-	-	-	-
%     \end{tabular}
%     % }
%     \caption{Performance on AVS (Single Source)}
%     \label{tab:ablation}
%     \vspace{-5pt}
% \end{table*}

% \usepackage{graphicx}
% \usepackage{multirow} 


\begin{table*}[t!]
\centering
\caption{Comparison of different fusion strategies and implementation of the method. We use D-ResNet50~\cite{he2016deep} and DeepLabV3+~\cite{chen2018encoder} as the backbone and the segmentation architecture.\yuanhong{move away}}
\resizebox{1.\linewidth}{!}{%
\begin{tabular}{!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccc|ccc|ccc!{\vrule width 1.5pt}} 
\specialrule{1.5pt}{0pt}{0pt}
\multirow{2}{*}{w/ sounds } & \multirow{2}{*}{Sum } & \multirow{2}{*}{Concate.} & \multirow{2}{*}{Att.} & \multirow{2}{*}{CAVP} & \multicolumn{3}{c|}{AVSBench-Semantic (SS)} & \multicolumn{3}{c|}{VPO-SS}  & \multicolumn{3}{c!{\vrule width 1.5pt}}{VPO-MS}\\ 
\cline{6-14}
\rule{0pt}{10pt}
& & & & & 
FDR $\downarrow$ & mIoU $\uparrow$ & F1 $\uparrow$ & 
FDR $\downarrow$ & mIoU $\uparrow$ & F1 $\uparrow$ & 
FDR $\downarrow$ & mIoU $\uparrow$ & F1 $\uparrow$ \\ 
\specialrule{1.5pt}{0pt}{0pt}
% \rowcolor{gray} 
\pmb{\tikzxmark} & & & & &     
15.56	&	68.11	&	80.37	&	26.11	&	50.10	&	64.12	&	21.56	&	50.37	&	64.28	\\
\textcolor{red}{\pmb{\tikzcmark}}&  \textcolor{red}{\pmb{\tikzcmark}} & & & &                   
14.81	&	69.61	&	81.47	&	25.84	&	56.46	&	69.25	&	28.00	&	57.42	&	70.05	\\
\textcolor{red}{\pmb{\tikzcmark}}& & \textcolor{red}{\pmb{\tikzcmark}} & & & 
15.25	&	69.05	&	81.13	&	23.62	&	52.66	&	64.93	&	21.17	&	57.50	&	70.49	\\
\textcolor{red}{\pmb{\tikzcmark}}& & & \textcolor{red}{\pmb{\tikzcmark}} & &
14.50	&	70.33	&	82.06	&	21.71	&	58.87	&	71.41	&	19.68	&	57.84	&	71.07	\\
\hline
% \rowcolor{LightCyan} 
\textcolor{red}{\pmb{\tikzcmark}}& & & \textcolor{red}{\pmb{\tikzcmark}} & \textcolor{red}{\pmb{\tikzcmark}} &  
\textbf{12.71}	&	\textbf{74.17}	&	\textbf{84.86}	&	\textbf{20.41}	&	\textbf{61.21}	&	\textbf{73.29}	&	\textbf{18.64}	&	\textbf{59.58}	&	\textbf{72.46}	\\
\specialrule{1.5pt}{0pt}{0pt}
\end{tabular}
\label{tab:ablation}
}
\vspace{-10pt}
\end{table*}






% \begin{table*}[t!]
% \centering
% \caption{Change w/o sounds}
% % \resizebox{.9\linewidth}{!}{%
% \begin{tabular}{!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccc|ccc!{\vrule width 1.5pt}} 
% \specialrule{1.5pt}{0pt}{0pt}
% \multirow{2}{*}{w/o sounds } & \multirow{2}{*}{Sum } & \multirow{2}{*}{Concate.} & \multirow{2}{*}{Att.} & \multirow{2}{*}{Contr.} & \multicolumn{3}{c|}{AVSBench-Single+} & \multicolumn{3}{c!{\vrule width 1.5pt}}{VPO-SS}  \\ 
% \cline{6-11}
% \rule{0pt}{10pt}
% & & & & & 
% FDR $\downarrow$ & mIoU $\uparrow$ & F1 $\uparrow$ & FDR $\downarrow$ & mIoU $\uparrow$ & F1 $\uparrow$ \\ 
% \specialrule{1.5pt}{0pt}{0pt}
% \textcolor{red}{\pmb{\tikzcmark}} & & & & &     
% 15.56	&	68.11	&	80.37	&	0	&	0	&	0	\\
% &  \textcolor{red}{\pmb{\tikzcmark}} & & & &                   
% 0	&	0	&	0	&	0	&	0	&	0	\\
% & & \textcolor{red}{\pmb{\tikzcmark}} & & & 
% 0	&	0	&	0	&	0	&	0	&	0	\\
% & & & \textcolor{red}{\pmb{\tikzcmark}} & &
% 15.50	&	70.33	&	82.06	&	0	&	0	&	0	\\       
% \rowcolor{LightCyan} & & & & \textcolor{red}{\pmb{\tikzcmark}} &     
% 12.71	&	74.17	&	84.86	&	0	&	0	&	0	\\
% \specialrule{1.5pt}{0pt}{0pt}
% \end{tabular}
% % }
% \end{table*}




==> table/avsbench_224.tex <==
\begin{table*}[!ht]
    \centering
    \caption{Quantitative (mIoU, $F_{\beta})$ audio-visual segmentation results (in \%) on AVSBench dataset~\cite{zhou2022audio,zhou2023audio} (resized to 224$\times$224) with ResNet50~\cite{he2016deep} and PVT-V2-B5~\cite{wang2022pvt} backbones. The best results are in \textbf{bold} and second-best,  \underline{underlined}. Improvements between our method and the second best are in brackets.}
    \vspace{-5pt}
    \label{tab:avsbench_224}
    % \def\arraystretch{1.1}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}c!{\vrule width 1.5pt}cc|cc|cc!{\vrule width 1.5pt}} 
\specialrule{1.5pt}{0pt}{0pt}
\multirow{2}{*}{\makecell{Architectural \\ (Backbone)}} & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{AVSBench-Object (SS)} & \multicolumn{2}{c|}{AVSBench-Object (MS)} & \multicolumn{2}{c!{\vrule width 1.5pt}}{AVSBench-Semantics} \\
\cline{3-8}
\rule{0pt}{10pt}
~ & ~ &  mIoU $\uparrow$ & $F_{\beta}$ $\uparrow$ &  mIoU $\uparrow$ & $F_{\beta}$ $\uparrow$ &  mIoU $\uparrow$ & $F_{\beta}$ $\uparrow$  \\ 
\specialrule{1.5pt}{0pt}{0pt}
% ---------
\multirow{6}{*}{\makecell{Transformer \\ (D-ResNet50~\cite{he2016deep})}} & CATR~\cite{li2023catr} & 74.80 & 86.60 & 52.80 & 65.30 & - & - \\ 
& AuTR~\cite{liu2023audio} & 75.00 & 85.20 & 49.40 & 61.20 & - & - \\ 
& AQFormer~\cite{huang2023discovering} & 77.00 & 86.40 & \underline{55.70} & \underline{66.90} & - & - \\ 
& AVSegFormer~\cite{gao2023avsegformer} & 76.54 & 84.80 & 49.53 & 62.80 & \underline{24.93} & 29.30 \\ 
& AVSC~\cite{liu2023audiovisual} & 77.02 & 85.24 & 49.58 & 61.51 & - & - \\ 
& BAVS~\cite{liu2023bavs} & \underline{77.96} & 85.29 & 50.23 & 62.37 & 24.68 & \underline{29.63} \\ \hline
\multirow{4}{*}{\makecell{Per-pixel Classification \\ (D-ResNet50~\cite{he2016deep})}} 
& TPAVI~\cite{zhou2022audio} & 72.79 & 84.80 & 47.88 & 57.80 & 20.18 & 25.20 \\ 
& AVSBG~\cite{hao2023improving} & 74.13 & 85.40 & 44.95 & 56.80 & - & - \\
& ECMVAE~\cite{mao2023multimodal} & 76.33 & 86.50 & 48.69 & 60.70 & - & - \\ 
& DiffusionAVS~\cite{mao2023contrastive} & 75.80 & \underline{86.90} & 49.77 & 62.10 & - & - \\ 
\rowcolor{LightCyan}\cellcolor{white}
% \cline{2-}
~ & \textbf{Ours} & \textbf{85.77}\tabgreen{+7.81} & \textbf{92.86}\tabgreen{+5.96} & \textbf{62.39}\tabgreen{+6.69} & \textbf{73.62}\tabgreen{+6.72} & \textbf{44.70}\tabgreen{+19.77} & \textbf{57.76}\tabgreen{+28.13} \\
% --------- 
\hline
%
%
%
%
%
%
\hline
\multirow{5}{*}{\makecell{Transformer \\ (PVT-V2-B5~\cite{wang2022pvt})}} 
& CATR~\cite{li2023catr} & 81.40 & 89.60 & 59.00 & 70.00 & 32.80 & 38.50 \\ 
& AuTR~\cite{liu2023audio} & 80.40 & 89.10 & 56.20 & 67.20 & - & - \\
& AQFormer~\cite{huang2023discovering} & 81.60 & 89.40 & \underline{61.10} & \underline{72.10} & - & - \\ 
& AVSegFormer~\cite{gao2023avsegformer} & \underline{82.06} & 89.90 & 58.36 & 69.30 & \underline{36.66} & \underline{42.00} \\ 
& AVSC~\cite{liu2023audiovisual} & 80.57 & 88.19 & 58.22 & 65.10 & - & - \\ 
& BAVS~\cite{liu2023bavs} & 81.96 & 88.60 & 58.63 & 65.49 & 32.64 & 36.42 \\ \hline
\multirow{4}{*}{\makecell{Per-pixel Classification \\ (PVT-V2-B5~\cite{wang2022pvt})}} 
& TPAVI~\cite{zhou2022audio} & 78.74 & 87.90 & 54.00 & 64.50 & 29.77 & 35.20 \\
& AVSBG~\cite{hao2023improving} & 81.71 & 90.40 & 55.10 & 66.80 & - & - \\
& ECMVAE~\cite{mao2023multimodal} & 81.74 & 90.10 & 57.84 & 70.80 & - & - \\ 
& DiffusionAVS~\cite{mao2023contrastive} & 81.38 & \underline{90.20} & 58.18 & 70.90 & - & - \\ 
\rowcolor{LightCyan}\cellcolor{white}
~ & \textbf{Ours} & \textbf{87.33}\tabgreen{+5.27} & \textbf{93.61}\tabgreen{+3.41} & \textbf{67.31}\tabgreen{+6.21} & \textbf{78.09}\tabgreen{+5.99} & \textbf{48.59}\tabgreen{+11.93} & \textbf{61.97}\tabgreen{+19.97} \\ 

\specialrule{1.5pt}{0pt}{0pt}
    \end{tabular}
}
\vspace{-10pt}
    
\end{table*}

==> table/avsbench_224_pvt.tex <==
\begin{table*}[!ht]
    \centering
    \caption{Quantitative (mIoU, $F_{\beta})$ audio-visual segmentation results (in \%) on AVSBench dataset~\cite{zhou2022audio,zhou2023audio} (resized to 224$\times$224) with PVT-V2-B5~\cite{wang2022pvt} backbone. The best results are in \textbf{bold} and the second best are \underline{underlined}.}
    \vspace{-5pt}
    \label{tab:avsbench_224_pvt}
    % \def\arraystretch{1.1}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}c!{\vrule width 1.5pt}cc|cc|cc!{\vrule width 1.5pt}} 
\specialrule{1.5pt}{0pt}{0pt}
\multirow{2}{*}{PVT-V2-B5~\cite{wang2022pvt}} & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{AVSBench-Object (SS)} & \multicolumn{2}{c|}{AVSBench-Object (MS)} & \multicolumn{2}{c!{\vrule width 1.5pt}}{AVSBench-Semantics} \\
\cline{3-8}
\rule{0pt}{10pt}
~ & ~ &  mIoU $\uparrow$ & $F_{\beta}$ $\uparrow$ &  mIoU $\uparrow$ & $F_{\beta}$ $\uparrow$ &  mIoU $\uparrow$ & $F_{\beta}$ $\uparrow$  \\ 
\specialrule{1.5pt}{0pt}{0pt}
% ---------
\multirow{5}{*}{Transformer} 
& CATR~\cite{li2023catr} & 81.40 & 89.60 & 59.00 & 70.00 & 32.80 & 38.50 \\ 
& AuTR~\cite{liu2023audio} & 80.40 & 89.10 & 56.20 & 67.20 & - & - \\
& AQFormer~\cite{huang2023discovering} & 81.60 & 89.40 & \underline{61.10} & \underline{72.10} & - & - \\ 
& AVSegFormer~\cite{gao2023avsegformer} & \underline{82.06} & 89.90 & 58.36 & 69.30 & \underline{36.66} & \underline{42.00} \\ 
& AVSC~\cite{liu2023audiovisual} & 80.57 & 88.19 & 58.22 & 65.10 & - & - \\ 
& BAVS~\cite{liu2023bavs} & 81.96 & 88.60 & 58.63 & 65.49 & 32.64 & 36.42 \\ \hline
\multirow{4}{*}{Per-pixel Classification} 
& TPAVI~\cite{zhou2022audio} & 78.74 & 87.90 & 54.00 & 64.50 & 29.77 & 35.20 \\
& AVSBG~\cite{hao2023improving} & 81.71 & 90.40 & 55.10 & 66.80 & - & - \\
& ECMVAE~\cite{mao2023multimodal} & 81.74 & 90.10 & 57.84 & 70.80 & - & - \\ 
& DiffusionAVS~\cite{mao2023contrastive} & 81.38 & \underline{90.20} & 58.18 & 70.90 & - & - \\ 
\rowcolor{LightCyan}\cellcolor{white}
~ & \textbf{Ours} & \textbf{87.33}\tabgreen{+5.27} & \textbf{93.61}\tabgreen{+3.41} & \textbf{67.31}\tabgreen{+6.21} & \textbf{78.09}\tabgreen{+5.99} & \textbf{48.59}\tabgreen{+11.93} & \textbf{61.97}\tabgreen{+19.97} \\ 
% --------- 
\specialrule{1.5pt}{0pt}{0pt}
    \end{tabular}
}
\vspace{-10pt}
    
\end{table*}

==> table/dataset_compare.tex <==

% \begin{table}[t]
% \begin{center}
% % \vspace{-1mm}
% \caption{\textbf{Existing audio-visual dataset statistics.}}
% % \begin{tabular}{l rrrr}
% \setlength{\tabcolsep}{6pt}
% \resizebox{1\linewidth}{!}{  
% \begin{tabular}{cccccc}
% \toprule[0.8pt]\noalign{\smallskip}


\begin{table*}
\centering
\caption{Comparison of recently published AVS datasets~\cite{hu2022mix,zhou2022audio} and our proposed 
VPO-SS, VPO-MS, and AVSBench-Single+ benchmark datasets, in terms of the number of samples, number of classes, sample type, annotation type, and if the audio-visual samples are synthesised.}
% \resizebox{1.\linewidth}{!}{%
\begin{tabular}{!{\vrule width 1.5pt}cccccc!{\vrule width 1.5pt}} 
\specialrule{1.5pt}{0pt}{0pt}

Benchmark & \# Samples & Classes & Types  &  Annotations & Synthesised?\\
% \noalign{\smallskip}
\specialrule{1.5pt}{0pt}{0pt}
% VGG-SS~\cite{chen2021localizing}         & \,\,\,5,158  & 220  & Image & BBox (Saliency)    \\  
VGG-Instruments~\cite{hu2022mix} & \,\,\,446  & \,\,\,37  & Image+Audio & Binary (Pixel) & \textcolor{red}{\pmb{\tikzxmark}}            \\
AVSBench-Objects-SS~\cite{zhou2022audio}        & 10,852 & \,\,\,23   & Video & Binary (Pixel) & \textcolor{red}{\pmb{\tikzxmark}}              \\
AVSBench-Objects-MS~\cite{zhou2022audio}        & 2,120 & \,\,\,23   & Video & Binary (Pixel) & \textcolor{red}{\pmb{\tikzxmark}}              \\
AVSBench-Semantics+ & 10,852 & \,\,\,23   & Video & Multi-class (Pixel) & \textcolor{red}{\pmb{\tikzxmark}}     
     \\
\rowcolor{LightCyan} VPO-SS & 12,202 & \,\,\,21   & Image+Audio & Multi-class (Pixel) & \textcolor{red}{\pmb{\tikzcmark}}               \\
\rowcolor{LightCyan} VPO-MS & 9,817 & \,\,\,21   & Image+Audio & Multi-class (Pixel) & \textcolor{red}{\pmb{\tikzcmark}}                \\

\specialrule{1.5pt}{0pt}{0pt}
\end{tabular}
% }
\label{tab:comparison_with_datasets}
\vspace{-10pt}
\end{table*}



% \bottomrule[0.8pt]
% \end{tabular}
% }
% \end{center}
% \vspace{-8mm}
% \end{table}
